Data-Driven Superstabilizing Control under Quadratically-Bounded Errors-in-Variables Noise

The Error-in-Variables model of system identification/control involves nontrivial input and measurement corruption of observed data, resulting in generically nonconvex optimization problems. This paper performs full-state-feedback stabilizing control of all discrete-time linear systems that are consistent with observed data for which the input and measurement noise obey quadratic bounds. Instances of such quadratic bounds include elementwise norm bounds (at each time sample), energy bounds (across the entire signal), and chance constraints arising from (sub)gaussian noise. Superstabilizing controllers are generated through the solution of a sum-of-squares hierarchy of semidefinite programs. A theorem of alternatives is employed to eliminate the input and measurement noise process, thus improving tractability.

==> sections/acknowledgements.tex <==
\section*{Acknowledgements}

We would like to thank Mohamed Abdalmoaty and Roy S. Smith for discussions about the Errors-in-Variables setting.

% \urg{Optional acknowledgements.}
% The authors thank Milan Korda for his discussions about occupation measures and time-varying uncertainty.

==> sections/contributions.tex <==

\urg{The contributions of this work are,
\begin{itemize}
    \item Contributions
    \item go
    \item here
\end{itemize}}

==> sections/extensions.tex <==
\section{Included Process Noise}
\label{sec:extensions}
Process noise can be added to the quadratically-bounded \ac{EIV} framework developed in this paper. Consider structured process noise $\{w_t\}$ corrupting dynamics in \eqref{eq:discrete_dynamics}, leading to the relation (with known $E \in \R^{n \times n_w}$)
\begin{equation}
        x_{t+1}= A x_t + B u_t + E w_t. \label{eq:discrete_dynamics_w}
\end{equation}
% Let $E^\dagger$ be a left inverse of $E$ ($E^\dagger E = I_{n_w}$) and $\Psi$ be a basis for the nullspace of $E$. 
The consistency set of plants $\bpc^w(A, B, \dx, \du, w)$ compatible with data in $\dc$ is
\begin{align}
    \bar{\pc}^w:=  \begin{Bmatrix*}[l]\Xi \dx + (I_{T-1} \otimes B) \du + (I_{T-1} \otimes E) w = -h^0  \\
       (F_\ell \dx + G_\ell \du + H_\ell w, 1)  \in \ls^{n_\ell}  \qquad  \forall \ell  \in 1..L\\
     \end{Bmatrix*}, \nonumber 
\end{align}
% \label{eq:pcbar_cone_w}
in which $\{H_\ell\}$ are matrices reflecting the quadratic constraints imposed on $w$.
The process-noise version of the constraint \eqref{eq:q_feas} is
\begin{align}
    \forall (A, B, \dx, \du, w) \in \bpc^w: & & q(A, B) \geq 0. \label{eq:q_feas_w}
\end{align}

A degree-$2k$ \ac{SOS} truncation of \eqref{eq:q_feas_w} can proceed directly by $q(A, B) \in \Sigma^1[\bpc^w]_{\leq 2k},$ yielding Gram matrices of size $\binom{n(n+T) + m(n+T-1)+n_w+k}{k}$.
The Theorem of Alternatives process eliminates the noise variables $(\dx, \du, w)$ altogether. The expression of \eqref{eq:q_feas_w} adds the following entry to the constraints in \eqref{eq:q_altern}:
\begin{align}
    (I_{T-1} \kron E^\tr) \mu + \textstyle \sum_{\ell=1}^L H_\ell^\tr s_\ell = 0.
\end{align}
Just like in the case without process noise, the infinite-dimensional linear constraints depend solely on $(A, B)$ after robustifying against noise, and the size of the maximal Gram matrices are found in \eqref{eq:size_altern} and \eqref{eq:size_block}.

% The known matrix  encodes the structure

% \urg{Process noise?}
